Dash: Scalable Hashing on Persistent Memory

Byte-addressable persistent memory (PM) brings hash tables the potential of low latency, cheap persistence and instant recovery. The recent advent of Intel Optane DC Persistent Memory Modules (DCPMM) further accelerates this trend. Many new hash table designs have been proposed, but most of them were based on emulation and perform sub-optimally on real PM. They were also piece-wise and partial solutions that side-step many important properties, in particular good scalability, high load factor and instant recovery. We present Dash, a holistic approach to building dynamic and scalable hash tables on real PM hardware with all the aforementioned properties. Based on Dash, we adapted two popular dynamic hashing schemes (extendible hashing and linear hashing). On a 24-core machine with Intel Optane DCPMM, we show that compared to state-of-the-art, Dash-enabled hash tables can achieve up to ~3.9X higher performance with up to over 90% load factor and an instant recovery time of 57ms regardless of data size.

==> dash-eh-search-helpers.tex <==
\begin{lstlisting}[language=python,
	mathescape,
	gobble=0,
	keywordstyle=\ttfamily\bfseries\color{blue},
	]
def bucket::search(key):
  h = hash(key)
  key_fp = LSB_byte(h)  # Generate fingerprint

  [fps, slot_ids] = get_matching_fingerprints(key_fp)
  for fp, slot_id in fps, slot_ids:
    slot = slots[slot_id]
    if slot.key == key:
      return slot.value
  return NULL
\end{lstlisting}

